SPARTA: Efficient Open-Domain Question Answering via Sparse Transformer Matching Retrieval

We introduce SPARTA, a novel neural retrieval method that shows great promise in performance, generalization, and interpretability for open-domain question answering. Unlike many neural ranking methods that use dense vector nearest neighbor search, SPARTA learns a sparse representation that can be efficiently implemented as an Inverted Index. The resulting representation enables scalable neural retrieval that does not require expensive approximate vector search and leads to better performance than its dense counterpart. We validated our approaches on 4 open-domain question answering (OpenQA) tasks and 11 retrieval question answering (ReQA) tasks. SPARTA achieves new state-of-the-art results across a variety of open-domain question answering tasks in both English and Chinese datasets, including open SQuAD, Natuarl Question, CMRC and etc. Analysis also confirms that the proposed method creates human interpretable representation and allows flexible control over the trade-off between performance and efficiency.

==> experiments.tex <==
In this section, we present the experiment setup for a proposed multi-domain ReQA task. 

\subsection{Multi-domain Retrieval Question Answering (MultiReQA)}

Retrieval Question Answering (ReQA) is a sentence-level extractive question answering task~\cite{ahmad2019reqa}. The candidate answer set contains every possible sentence from a text corpus and the system is expected to return a ranking of answer sentences given a question. The original ReQA only contains SQuAD~\cite{rajpurkar2016squad} and Natural Question~\cite{kwiatkowski2019natural}. In this study, we extend ReQA to 11 different domains adapted from~\cite{fisch2019mrqa} to evaluate various methods for both \textit{in-domain performance} and \textit{out-of-domain generalization}. The details of the 11 ReQA domains are in Table~\ref{tbl:reqa_data} and Table~\ref{tbl:reqa_size}.

Each of these domains originally comes in the format of SQuAD 1.1~\cite{fisch2019mrqa}. We use NLTK sentence splitter~\cite{loper2002nltk} to segment all paragraphs into sentences. Each sentence is treated as a candidate answer. Moreover, we keep the surrounding context words of each candidate answer as its context $c$. We encode at most 512 word piece tokens and truncate the context surrounding the answer sentence with equal window size. For model training, \textit{bert-base-uncased} is used as the answer encoder. We reuse the word embedding from bert-base-uncased as the term embedding and keep them fixed during training. Adam~\cite{kingma2014adam} is used as the optimizer for fine-tuning with a learning rate 3e-5. The model is fine-tuned for at most 10K steps and the best model is picked based on MRR performance based on held-out validation datasets. 

The in-domain scenarios focus on domains that have enough training data (see Table~\ref{tbl:reqa_data}). The models are trained on the training data and the evaluation is done on the corresponding test data. On the other hand, the out-of-domain scenarios evaluate systems' performance on test data from domains not included in the training, making it a zero-shot learning problem. There are two out-of-domain settings: (1) training data only contain SQuAD (2) training data contain only SQuAD and NQ. Evaluation is carried on all the domains to test systems' ability to generalize to unseen data distribution.

\begin{table}[ht]
\small
\begin{tabular}{p{0.28\textwidth}p{0.16\textwidth}} \hline
\textbf{Domain}                        & \textbf{Data Source}  \\ \hline
Has training data & \\ \hline
SQuAD~\cite{rajpurkar2016squad}          & Wikipedia                    \\
News~\cite{trischler2016newsqa}          & News                       \\
Trivia~\cite{joshi2017triviaqa}          & Web                        \\
NQ~\cite{kwiatkowski2019natural}         & Google Search                                           \\
Hotpot~\cite{yang2018hotpotqa}           & Wikipedia                       \\ \hline
Has no training data                    &                              \\ \hline
BioASQ~\cite{tsatsaronis2015overview}    & PubMed Documents                  \\
DROP~\cite{dua2019drop}                  & Wikipedia                       \\
DuoRC~\cite{saha2018duorc}               & Wikipedia+IMDB                       \\
RACE~\cite{lai2017race}                  & English Exam                       \\
RE~\cite{levy2017zero}                   & Wikipedia                       \\
Textbook~\cite{kembhavi2017you}          & K12 Textbook                  \\ \hline
\end{tabular}
\caption{11 corpora included in MultiReQA and their document sources. The top 5 domains contain training data and the bottom 6 domains only have test sets.}
\label{tbl:reqa_data}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{p{0.1\textwidth}|p{0.12\textwidth}p{0.2\textwidth}} \hline
\textbf{Domain}                        & \textbf{\# of Query}  & \textbf{\# of Candidate Answer} \\ \hline
SQuAD         & 11,426  & 10,250                    \\
News          & 8,633        &38,199               \\
Trivia          & 8,149  & 17,845                        \\
NQ       & 1,772  &  7,020                \\
Hotpot          & 5,901      & 38,906                 \\ 
BioASQ   & 1,562  & 13,802                  \\
DROP                  & 1,513  & 2,488                       \\
DuoRC          & 1,568  & 5,241                  \\
RACE                  & 674  & 10,630                   \\
RE                   & 2,947  & 2,201                       \\
Textbook          &  1,503  & 14,831                  \\ \hline
\end{tabular}
\caption{Size of the evaluation test set for the 11 corpora included in MultiReQA.}
\label{tbl:reqa_size}
\end{table}

For evaluation metrics, we use \textit{Mean Reciprocal Rank} (MRR) as the criteria. The competing baselines include:
\begin{itemize}
    \item BM25: a proven strong classic IR baseline that is difficult to beat~\cite{robertson2009probabilistic}.
    \item USE-QA\footnote{\url{https://tfhub.dev/google/universal-sentence-encoder-multilingual-qa}}: universal sentence encoder trained for QA task by Google~\cite{yang2019multilingual}. USE-QA uses the dual-encoder architecture and it is trained on more than 900 million mined question-answer pairs with 16 different languages. 
    \item Poly-Encoder (Poly-Enc): Poly Encoders improves the expressiveness of dual-encoders with two-level interaction~\cite{humeau2019poly}. The original implementation is for dialog response ranking so we adapted it for question answering retrieval. Specifically, two bert-base-uncased models are used as the question and answer encoders. The answer encoder outputs 4 vectors instead of 1 vector as the answer representations.
\end{itemize}

\subsection{Open-domain Question Answering (OpenQA)}
We also consider an Open-domain Question Answering (OpenQA) task to evaluate the performance of SPARTA ranker. Following previous work on OpenQA \cite{chen2017reading, wang2019multi, xie2020distant}, we experiment with two English datasets (SQuAD~\cite{rajpurkar2016squad}, NQ~\cite{kwiatkowski2019natural}) and two Chinese datasets (CMRC~\cite{cui2018span}, DRCD~\cite{shao2018drcd}) and compare the results with previous OpenQA models.

For each dataset, we follow the original version of Wikipedia where the data was collected from, and dump as the text knowledge base. We then index every sentence in the data as candidate answers. 

In order to extract phrase-level span as required by OpenQA task, we use a pre-trained MRC reader based on SpanBERT~\cite{joshi2020spanbert} to extract answer phrases from the top-K returned sentences. To make the span answer score comparable among different passages, we use global normalization ~\cite{clark2017simple}, which normalizes span scores among multiple passages. Also, distant supervision is used in the MRC model to make the training distribution more close to test distribution, as discussed in ~\cite{xie2020distant}.


Evaluation metrics include the standard SQuAD metric: EM F1-score and Recall:

\begin{itemize}
    \item Exact Match (EM): if the top-1 answer span matches with the ground truth exactly.
    \item F1 Score: we compute word overlapping between the returned span and the ground truth answer at token level.
    \item Recall (R): we consider it a successful prediction if the ground truth answer can be found in the top-K retrieved sentences.
\end{itemize}



==> results.tex <==
\subsection{MultiReQA Results}
\subsubsection{In-domain Performance}
\begin{table}[]
\centering
\begin{tabular}{p{0.07\textwidth}|p{0.07\textwidth}p{0.07\textwidth}p{0.07\textwidth}p{0.07\textwidth}} \hline
\textbf{Data} & \textbf{BM25} & \textbf{USE-QA} & \textbf{Poly Enc} & \textbf{SPARTA (ours)}\\ \hline
SQuAD  & 58.0 & 62.5   & 64.6     & \textbf{78.5}   \\
News   & 19.4 & 26.2 & 28.3     & \textbf{46.6}  \\
Trivia & 29.0   & 41.2   & 39.5     & \textbf{55.5}   \\
NQ     & 19.7 & 58.2   & 69.9     & \textbf{77.1}   \\
HotPot & 23.9 & 25.5   & 51.8     & \textbf{63.8}  \\ \hline
Avg    & 30.0 &  42.7  &  50.8  & \textbf{64.3} \\ \hline
\end{tabular}
\caption{MRR comparison for the in-domain settings. The proposed SPARTA consistently outperforms all the baseline models with large margin. BM25 and USE-QA are unsupervised and pre-trained respectively.}
\label{tbl:in-domain}
\end{table}

\begin{table*}[!ht]
\centering
\small
\begin{tabular}[width=16cm]{l|lllll|llllll|l} \hline
 \textbf{Model}   & \textbf{SQuAD} & \textbf{News}  & \textbf{Trivia} & \textbf{NQ}    & \textbf{HotPot} & \textbf{Bio}   & \textbf{DROP}  & \textbf{DuoRC} & \textbf{RACE}  & \textbf{RE}    & \textbf{Text}  & \textbf{Avg}   \\ \hline
 & \multicolumn{12}{c}{Unsupervised or pretrained}                                              \\ \hline
BM25      & 58.0 & 19.4 & 29.0  & 19.7  & 23.9  & 8.9 & 32.6 & 20.1 & 14.8 & 87.4 & 21.6 & 30.5 \\
USE-QA    & 62.5 & 26.2 & 41.2  & 58.2 & 25.5  & 7.7 & 31.9 & 20.8 & 25.6 & 84.8 & 26.4 & 37.4 \\ \hline
          & \multicolumn{12}{c}{Trained on SQuAD}                                              \\ \hline
PolyEnc & 64.6* & 22.2 & 35.9  & 57.6 & 26.5  & 9.1 & 32.6 & 25.4 & 24.7 & 88.3 & 26.0 & 37.5  \\
SPARTA    & 78.5* & \textbf{41.2} & 45.8  & 62.0 & \textbf{47.7}  & 14.5 & 37.2 & 35.9 & 29.7 & 96.0& 28.7 & 47.0 \\\hline
          & \multicolumn{12}{c}{Trained on SQuAD + NQ}                                              \\ \hline
PolyEnc & 63.9* & 19.8 & 36.9  & 69.7* & 29.6  & 8.8 & 30.7 & 19.6 & 25.2 & 72.8 & 24.6 & 36.5 \\
SPARTA    &\textbf{79.0}*  & 40.3  & \textbf{47.6} & \textbf{75.8}*  & 47.5 & \textbf{15.0} &\textbf{ 37.9} & \textbf{36.3} & \textbf{30.0} & \textbf{97.0} & \textbf{29.3} & \textbf{48.7} \\\hline
\end{tabular}
\caption{MRR comparison in the out-of-domain settings. The proposed SPARTA is able to achieve the best performance across all tasks, the only learning-based method that is able to consistently outperform BM25 with larger margin in new domains. Results with * are in-domain performance.}
\label{tbl:out-domain}
\end{table*}

Table~\ref{tbl:in-domain} shows the MRR results on the five datasets with in-domain training. SPARTA can achieve the best performance across all domains with a large main. In terms of average MRR across the five domains, SPARTA is 114.3\% better than BM25, 50.6\% better than USE-QA and 26.5\% better than Poly-Encoders. 

Two additional insights can be drawn from the results. First, BM-25 is a strong baseline and does not require training. It performs particularly well in domains that have a high-rate of word-overlapping between the answer and the questions. For example, SQuAD's questions are generated by crowd workers who look at the ground truth answer, while question data from NQ/News are generated by question makers who do not see the correct answer. BM25 works particularly well in SQuAD while performing the poorest in other datasets. Similar observations are also found in prior research~\cite{ahmad2019reqa}.

Second, the results in Table~\ref{tbl:in-domain} confirms our hypothesis on the importance of rich interaction between the answer and the questions. Both USE-QA and Poly Encoder use powerful transformers to encode the whole question and model word-order information in the queries. However, their performance is bounded by the simple dot-product interaction between the query and the answer. On the other hand, despite the fact that SPARTA does not model word-order information in the query, it is able to achieve a big performance gain compared to the baselines, confirming the effectiveness of the proposed token-level interaction method in Eq.~\ref{eq:term_match}.


\subsubsection{Out-of-domain Generalization}
Table~\ref{tbl:out-domain} summarized the results for out-of-domain performance comparison. SPARTA trained only on SQuAD outperforms the baselines, achieving 54.1\% gain compared to BM25, 26.7\% gain compared to USE-QA and 25.3\% gain compared to Poly-Encoders in terms of average MRR across 11 different datasets. When SPARTA is trained on SQuAD+NQ, an additional 1.7 MRR improvement is gained compared to SPARTA-SQuAD. 

\begin{table}[ht]
\centering
\begin{tabular}{l|ll} \hline
\textbf{Setting}  & \textbf{Poly-Encoder} & \textbf{SPARTA} \\ \hline
\multicolumn{3}{c}{Trained on SQuAD}                                  \\ \hline
In-domain  & 47.4                        & 60.8                       \\
Out-domain & 35.6                        & 49.2                       \\
Diff       & -25.0\%                     & -19.2\%                    \\ \hline
\multicolumn{3}{c}{Trained on SQuAD+NQ}                               \\ \hline
In-domain  & 39.9                        & 55.3                      \\
Out-domain & 28.8                        & 45.1                       \\
Diff       & -29.2\%                     & -18.3\%                    \\ \hline
\end{tabular}
\caption{Average performance drop compared between in-domain and out-of-domain settings. For models trained on SQuAD, the included domains are: News, Trivia, NQ and Hotpot. For models trained SQuAD+NQ, the included domains are: News, Trivia and Hotpot. }
\label{tbl:diff}
\end{table}

We also note several key observations by investigating detailed performance differences in each domain.

\textbf{SPARTA generalizes better in new domains} We can observe that Poly-Encoder is able to achieve similar in-domain performance for the domains that are included in the training. However, its performance decreases significantly in new domains, a 25.0\% drop compared to its full performance for Poly-Encoder that is trained on SQuAD and 29.2\% drop when it's trained on SQuAD+NQ. 

Meanwhile, SPARTA generalizes its knowledge from the training data much better to new domains. When trained on SQuAD, its performance on News, Trivia, NQ, and HotPot is only 19.2\% lower than the full performance and 18.3\% drop when it's trained on SQuAD+NQ. The above results are summarized in Table~\ref{tbl:diff}. Also, we note that SPARTA's zero-shot performance on News (MRR=41.2) and Trivia (MRR=45.8) is even better than the full performance of Poly-Encoder (News MRR=28.3 and Trivia MRR=39.5). 

\textbf{SPARTA benefits more from multi-task learning.} Table~\ref{tbl:out-domain} also shows by training on more data, e.g., SQuAD+NQ, SPARTA's performance for most of the datasets continues to increase, i.e., the average MRR increases from 47.0 to 48.7. 

The performance of Poly-Encoder, however, decreases after training on more data, especially for out-of-domain datasets. Despite extensive hyper-parameter tuning,  Poly-Encoder's average MRR drops from 37.5 to 36.5 in the multi-task setting. We argue that this is due to the limited expressiveness of sequence-level dot product, which makes Poly-Encoder struggle to learn a diverse set of matching behavior from different domains.  

%\subsection{Open-domain QA Results}

%\begin{table}[ht]
%\centering
%\small
%\begin{tabular}{l|lll} \hline
%\textbf{Model}                      & \textbf{EM} & \textbf{F1} & \textbf{R} \\ \hline
%Dr.QA                         &    &    &   \\
%Dr.QA +Multitask              &    &    &   \\
%R3                            &    &    &   \\
%MINMAL                        &    &    &   \\
%BERTserini (paragraph, k=100) &    &    &   \\ \hline
%SPARTA (k=10)                 &    &    &   \\
%SPARTA (k=100)                &    &    &   \\ \hline
%\end{tabular}
%\caption{Open-domain QA evaluation results on SQuAD. The latest Wikipedia dump is used as the %text knowledge base.}
%\label{tbl:open-qa}
%\end{table}

%Table~\ref{tbl:open-qa} summarizes results for open-domain question answering. 

\subsection{OpenQA Results}

% \begin{table*}[!ht]
% \centering
% \small
% \begin{tabular}[width=16cm]{l|cccc|cccc} \hline
%  \textbf{Model}   & \multicolumn{2}{c}{\textbf{OpenSQuAD}} & \multicolumn{2}{c}{\textbf{OpenNQ}}  & \multicolumn{2}{c}{\textbf{OpenCMRC}} & \multicolumn{2}{c}{\textbf{OpenDRCD}}  \\ \hline
% %   & \multicolumn{12}{c}{F1}           \\ \hline
% & F1 & EM & F1-dev & F1-test & F1 & EM & F1 & EM \\ \hline

% Dr.QA\cite{chen2017reading}  & - & 29.8 & - & -& -&-& -&-  \\ 
% R\textsuperscript{3} \cite{wang2018r}  & 37.5 & 29.1 & - & -& -&-& -&-  \\ 

% \end{tabular}
% \caption{OpenQA results for both English and Chinese Datasets}
% \label{tbl:out-domain}
% \end{table*}

Table \ref{tbl:openqa-en} and \ref{tbl:openqa-zh} shows the SPARTA performance in OpenQA settings, tested in both English and Chinese datasets. Experimental results show that SPARTA retriever outperforms all existing models and get state-of-the-art results on all four datasets. %% ADD more here

\begin{table}[]
\centering
\begin{tabular}{p{0.32\textwidth}p{0.05\textwidth}p{0.05\textwidth}} 
\hline
\textbf{OpenSQuAD} &  &  \\ 
Model & F1 & EM \\ \hline
Dr.QA\cite{chen2017reading}  & - & 29.8  \\ 
R\textsuperscript{3} \cite{wang2018r} & 37.5 & 29.1 \\
Par. ranker \cite{lee2018ranking} & - & 30.2 \\
MINIMAL \cite{min2018efficient} & 42.5 & 32.7 \\
DenSPI-hybrid \cite{seo2019real} & 44.4 & 36.2 \\
BERTserini \cite{yang2019end} & 46.1 & 38.6 \\
RE \textsuperscript{3} \cite{hu2019retrieve} & 50.2 & 41.9 \\
Multi-passage \cite{wang2019multi} & 60.9 & 53.0 \\
Graph-retriever \cite{asai2019learning} & 63.8 & 56.5 \\
\hline
SPARTA & \textbf{66.5} & \textbf{59.3} \\

\Xhline{3\arrayrulewidth}

\textbf{OpenNQ} & \multicolumn{2}{c}{F1} \\ 
Model & Dev & Test \\ \hline
BERT + BM25 \cite{lee2018ranking} & 24.8 & 26.5 \\
Hard EM \cite{min2019discrete} & 28.8 & 28.1\\
ORQA\cite{lee2019latent}  & 31.3 & 33.3  \\
Graph-retriever \cite{asai2019learning} & 31.7 & 32.6 \\
\hline
SPARTA & \textbf{36.8} & \textbf{37.5} \\
\hline

% \Xhline{3\arrayrulewidth}
\end{tabular}
\caption{OpenQA results on two English datasets}
\label{tbl:openqa-en}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{p{0.32\textwidth}p{0.05\textwidth}p{0.05\textwidth}} 
\hline
\textbf{OpenCMRC} &  &  \\ 
Model & F1 & EM \\ \hline
BERTserini\cite{xie2020distant} & 60.9 & 44.5 \\
BERTserini+DS \cite{xie2020distant} & 64.6 & 48.6 \\

\hline
SPARTA & \textbf{79.9} & \textbf{62.9} \\

\Xhline{3\arrayrulewidth}

\textbf{OpenDRCD} &  &  \\ 
Model & F1 & EM \\ \hline
BERTserini \cite{xie2020distant} & 65.0 & 50.7 \\
BERTserini+DS \cite{xie2020distant} & 67.7 & 55.4 \\
\hline
SPARTA & \textbf{74.6} & \textbf{63.1} \\
\hline

% \Xhline{3\arrayrulewidth}
\end{tabular}
\caption{OpenQA results on two Chinese datasets}
\label{tbl:openqa-zh}
\end{table}


